Interpretable Self-supervised Multi-task Learning for COVID-19 Information Retrieval and Extraction

The rapidly evolving literature of COVID-19 related articles makes it challenging for NLP models to be effectively trained for information retrieval and extraction with the corresponding labeled data that follows the current distribution of the pandemic. On the other hand, due to the uncertainty of the situation, human experts' supervision would always be required to double check the decision making of these models highlighting the importance of interpretability. In the light of these challenges, this study proposes an interpretable self-supervised multi-task learning model to jointly and effectively tackle the tasks of information retrieval (IR) and extraction (IE) during the current emergency health crisis situation. Our results show that our model effectively leverage the multi-task and self-supervised learning to improve generalization, data efficiency and robustness to the ongoing dataset shift problem. Our model outperforms baselines in IE and IR tasks, respectively by micro-f score of 0.08 (LCA-F score of 0.05), and MAP of 0.05 on average. In IE the zero- and few-shot learning performances are on average 0.32 and 0.19 micro-f score higher than those of the baselines.

==> 0_table.tex <==
\begin{table}
\centering
% \scriptsize
\begin{tabular}{l|c c c}
\hline
\multirow{2}{40pt}{\textbf{Dataset}} & \textbf{No. of} & \textbf{No. of} & \textbf{No. of Supp.} \\ 
 & \textbf{Documents} & \textbf{MeSH Indexes} & \textbf{Concepts} \\ \hline 
\multirow{2}{40pt}{\textbf{COVID SSL}} & \multirow{2}{15pt}{141,764} & \multirow{2}{15pt}{-} & \multirow{2}{15pt}{-} \\ 
& & & \\ \hline
\multirow{2}{40pt}{\textbf{BioASQ}} & \multirow{2}{15pt}{2,501,982} & 27,114 & - \\
     &   & (12.84/doc.) &  \\ \hline
\multirow{2}{40pt}{\textbf{COVID Train}} & \multirow{2}{15pt}{10,210} & 14,335 & 18 \\
     &   & (16.6/doc.) & (1.97/doc.) \\ \hline
\multirow{2}{40pt}{\textbf{COVID Test}} & \multirow{2}{15pt}{3,463} & 10,922 & 15 \\
     &   & (17.9/doc.) & (1.92/doc.) \\ \hline
\end{tabular}
\caption{Data Descriptive for selfsupervised representation learning and supervised extraction of semantic indexes (training and evaluation) datasets.} %%%
\label{table:data_desc}
\end{table}

==> 1_new_introduction.tex <==
The pandemic has resulted in a rapidly evolving literature of scientific publications regarding the novel coronavirus which has caused an information crisis \citep{roberts2020trec}. The researchers, healthcare practitioners, policy makers and other individuals fighting against COVID-19 require specialized information retrieval and extraction systems to keep up with the literature \citep{esteva2020co,wang2020covid}. In this regard, many models are proposed based on state-of-the-art natural language processing (NLP) techniques, including neural ranking models for document retrieval \citep{zhang2020covidex,esteva2020co,koksal2020vapur}, and pre-trained transformers for automated annotation and information extraction \citep{colic2020annotating,lymperopoulos2020concept,spangher2020enabling}.
% \citep{das2020information,verspoor2020covid,wang,trec,cord,allenai}

The focus of the literature has drastically shifted towards COVID-19 related topics causing a covariate shift problem.



On the other hand, the limited amount of labeled data and drastic changes of COVID-19 landscape \cite{shokraneh2020lessons} has made it challenging for such models to effectively scale up to the domain-specific environment of the current pandemic. 



During the current pandemic so many related papers are being published at a much faster pace,\cite{esteva2020co} and the focus of the literature has drastically shifted towards COVID-19 related topics and subtopics,\cite{roberts2020trec} some of them have not had a standard name until a couple of month ago.



A pandemic situation, however, is an extreme scenario which highlights the importance of automated semantic indexing as researchers desperately require a well compartmentalized database to gain insights about the recent findings.\cite{shokraneh2020lessons} 

Such conditions cause challenges for the automatic semantic indexing systems which are based on substantial supervisions and hand-coded features. Albeit the importance of semantic indexing in the pandemic situation, there is a lack of study on the performance of such automated models on the rapidly evolving corpus of COVID-19 related documents.\cite{shokraneh2020lessons}
